An Empirical Study of In-context Learning in LLMs for Machine Translation

Recent interest has surged in employing Large Language Models (LLMs) for machine translation (MT) via in-context learning (ICL) (Vilar et al., 2023). Most prior studies primarily focus on optimizing translation quality, with limited attention to understanding the specific aspects of ICL that influence the said quality. To this end, we perform the first of its kind, an exhaustive study of in-context learning for machine translation. We first establish that ICL is primarily example-driven and not instruction-driven. Following this, we conduct an extensive exploration of various aspects of the examples to understand their influence on downstream performance. Our analysis includes factors such as quality and quantity of demonstrations, spatial proximity, and source versus target originality. Further, we also investigate challenging scenarios involving indirectness and misalignment of examples to understand the limits of ICL. While we establish the significance of the quality of the target distribution over the source distribution of demonstrations, we further observe that perturbations sometimes act as regularizers, resulting in performance improvements. Surprisingly, ICL does not necessitate examples from the same task, and a related task with the same target distribution proves sufficient. We hope that our study acts as a guiding resource for considerations in utilizing ICL for MT. Our code is available on https://github.com/PranjalChitale/in-context-mt-analysis.

==> content/figures.tex <==
% bloom 1-shot
\begin{figure*}[h]
    \centering
    
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-legend.png}
    \end{subfigure}

    \vspace{0.5em}
    
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-en-xx-source-1shot-results.pdf}
        \caption{En-XX (Source) - 1 shot}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-en-xx-target-1shot-results.pdf}
        \caption{En-XX (Target) - 1 shot}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-xx-en-source-1shot-results.pdf}
        \caption{XX-En (Source) - 1 shot}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-xx-en-target-1shot-results.pdf}
        \caption{XX-En (Target) - 1 shot}
    \end{subfigure}

    \caption{Variation in ChrF++ scores across different attack types observed in BLOOM-7B derivatives when prompted in a 1-shot manner.}
    \label{fig:bloom-1shot}
\end{figure*}



% bloom 4-shot
\begin{figure*}[h]
    \centering
    
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-legend.png}
    \end{subfigure}

    \vspace{0.5em}
    
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-en-xx-source-4shot-results.pdf}
        \caption{En-XX (Source) - 4 shot}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-en-xx-target-4shot-results.pdf}
        \caption{En-XX (Target) - 4 shot}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-xx-en-source-4shot-results.pdf}
        \caption{XX-En (Source) - 4 shot}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-xx-en-target-4shot-results.pdf}
        \caption{XX-En (Target) - 4 shot}
    \end{subfigure}

    \caption{Variation in ChrF++ scores across different attack types observed in BLOOM-7B derivatives when prompted in a 4-shot manner.}
    \label{fig:bloom-4shot}
\end{figure*}



% bloom 8-shot
\begin{figure*}[h]
    \centering
    
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-legend.png}
    \end{subfigure}

    \vspace{0.5em}
    
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-en-xx-source-8shot-results.pdf}
        \caption{En-XX (Source) - 8 shot}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-en-xx-target-8shot-results.pdf}
        \caption{En-XX (Target) - 8 shot}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-xx-en-source-8shot-results.pdf}
        \caption{XX-En (Source) - 8 shot}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bloom-xx-en-target-8shot-results.pdf}
        \caption{XX-En (Target) - 8 shot}
    \end{subfigure}

    \caption{Variation in ChrF++ scores across different attack types observed in BLOOM-7B derivatives when prompted in a 8-shot manner.}
    \label{fig:bloom-8shot}
\end{figure*}



% llama 1-shot
\begin{figure*}[h]
    \centering
    
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-legend.png}
    \end{subfigure}

    \vspace{0.5em}
    
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-en-xx-source-1shot-results.pdf}
        \caption{En-X - 1 shot - source}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-en-xx-target-1shot-results.pdf}
        \caption{En-X - 1 shot - target)}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-xx-en-source-1shot-results.pdf}
        \caption{X-En - 1 shot - Source}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-xx-en-target-1shot-results.pdf}
        \caption{X-En 1-shot Target}
    \end{subfigure}

    \caption{Variation in ChrF++ scores across different attack types observed in Llama2-7B derivatives when prompted in a 1-shot manner.}
    \label{fig:llama-1shot}
\end{figure*}



% llama 4-shot
\begin{figure*}[h]
    \centering
    
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-legend.png}
    \end{subfigure}

    \vspace{0.5em}
    
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-en-xx-source-4shot-results.pdf}
        \caption{En-X - 4 shot - source}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-en-xx-target-4shot-results.pdf}
        \caption{En-X - 4 shot - target)}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-xx-en-source-4shot-results.pdf}
        \caption{X-En - 4 shot - Source}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-xx-en-target-4shot-results.pdf}
        \caption{X-En 4-shot Target}
    \end{subfigure}

    \caption{Variation in ChrF++ scores across different attack types observed in Llama2-7B derivatives when prompted in a 4-shot manner.}
    \label{fig:llama-4shot}
\end{figure*}



% llama 8-shot
\begin{figure*}[h]
    \centering
    
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-legend.png}
    \end{subfigure}

    \vspace{0.5em}
    
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-en-xx-source-8shot-results.pdf}
        \caption{En-X - 8 shot - source}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-en-xx-target-8shot-results.pdf}
        \caption{En-X - 8 shot - target)}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-xx-en-source-8shot-results.pdf}
        \caption{X-En - 8 shot - Source}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama-xx-en-target-8shot-results.pdf}
        \caption{X-En 8-shot Target}
    \end{subfigure}

    \caption{Variation in ChrF++ scores across different attack types observed in Llama2-7B derivatives when prompted in a 8-shot manner.}
    \label{fig:llama-8shot}
\end{figure*}

